Two variable logic with ultimately periodic counting

We consider the extension of two variable logic with quantifiers that state that the number of elements where a formula holds should belong to a given ultimately periodic set. We show that both satisfiability and finite satisfiability of the logic are decidable. We also show that the spectrum of any sentence is definable in Presburger arithmetic. In the process we present several refinements to the ``biregular graph method''. In this method, decidability issues concerning two-variable logics are reduced to questions about Presburger definability of integer vectors associated with partitioned graphs, where nodes in a partition satisfy certain constraints on their in- and out-degrees.

==> app-infinite-sec8.tex <==
%!TEX root = fo2siam.tex


\section{The extension of Section~\ref{sec:complexity} to the general case}
\label{app:sec:complexity}

In this appendix we will discuss the extension of the complexity analysis in Section ~\ref{sec:complexity}
to the general case.

\subsection{Complexity of the graph analysis}
\label{app:subsec:complexity-bireg}

In this subsection we extend the analysis in Subsection ~\ref{subsec:complexity-bireg}
to the general case, as stated as Lemma~\ref{app:lem:algo-for-bireg} and~\ref{app:lem:algo-for-direg}.
Here we simply note that the number of (in)equations for the general case remains the same, i.e., 
$O(2^tt^4\delta(A,B)^4)$ (in)equations. See Remark~\ref{app:rem:simple-complete}.
Thus, we omit the details of the proof.


\begin{lemma}
\label{app:lem:algo-for-bireg}
There is a non-deterministic Turing machine $\cM$ that does the following.
On input degree matrices $A\in \bbN_{\infty,+p}^{t\times m}$ and $B\in \bbN_{\infty,+p}^{t\times n}$,
on every run $r$ of $\cM$, it outputs an existential Presburger formula $\varphi_r(\vx,\vy)$ 
such that the following holds:
\begin{itemize}
\item 
each $\varphi_r(\vx,\vy)$ is of the form
$\exists\vz\ \widetilde{\varphi}_r(\vx,\vy,\vz)$,
where each $\widetilde{\varphi}_r(\vx,\vy,\vz)$ is a conjunction of $O(mn2^tt^4\delta(A,B)^4)$ linear (in)equations;
\item
for every $(\vM,\vN)\in \bbN^m\times \bbN^n$, 
there is complete $A|B$-biregular graph with size $\vM|\vN$
if and only if 
there is a run $r$ of $\cM$ such that $\varphi_r(\vM,\vN)$ holds in $\cN_{\infty}$.
\end{itemize}
Moreover, $\cM$ runs in time exponential in the size of $A$ and $B$,
where the coefficients of the input degree matrices and the output formula $\varphi_r$ are in binary.
\end{lemma}

\begin{lemma}
\label{app:lem:algo-for-direg}
There is a non-deterministic Turing machine $\cM$ that does the following.
On input degree matrices $A\in \bbN_{\infty,+p}^{t\times m}$ and $B\in \bbN_{\infty,+p}^{t\times m}$,
on every run $r$ of $\cM$, it outputs an existential Presburger formula $\varphi_r(\vx)$ 
such that the following holds:
\begin{itemize}
\item 
each $\varphi_r(\vx)$ is of the form $\exists\vz\ \widetilde{\varphi}_r(\vx,\vz)$,
where each $\widetilde{\varphi}_r(\vx,\vz)$ is a conjunction of $O(m^22^tt^4\delta(A,B)^4)$ linear (in)equations;
\item
for every $\vM\in \bbNo^m$, 
there is complete $A|B$-regular digraph with size $\vM$
if and only if 
there is a run $r$ of $\cM$ such that $\varphi_r(\vM)$ holds in $\cN_{\infty}$.
\end{itemize}
Moreover, $\cM$ runs in time exponential in the size of $A$ and $B$,
where the coefficients of the input degree matrices and the output formula $\varphi_r$ are in binary.
\end{lemma}

\subsection{2-$\nexp$ algorithm for the general satisfiability of $\fotwopres$}
\label{app:subsec:complexity-dec-proc}


The complexity analysis of the general satisfiability of $\fotwopres$ is almost the same as 
in Section ~\ref{subsec:complexity-dec-proc}.
The only difference is that the co-domain of a behavior function $g:\TwoTypes^*\times\OneTypes \to \bbNop$
is $\{\infty, 0,\ldots,q,\prdp{0},\ldots,\prdp{q}\}$,
where $q$ is the maximal (non $\infty$) offset in the u.p.s. $S_i$'s. 
Thus, asymptotically the total number of behavior functions is still the same.
Since the total number of (in)equations is still the same as the finite satisfiability case
the $2$-$\nexp$ upper bound also follows immediately for the general satisfiability of $\fotwopres$.


